Towards near-term quantum simulation of materials

Simulation of materials is one of the most promising applications of quantum computers. On near-term hardware the crucial constraint on these simulations is circuit depth. Many quantum simulation algorithms rely on a layer of unitary evolutions generated by each term in a Hamiltonian. This appears in time-dynamics as a single Trotter step, and in variational quantum eigensolvers under the Hamiltonian variational ansatz as a single ansatz layer. We present a new quantum algorithm design for materials modelling where the depth of a layer is independent of the system size. This design takes advantage of the locality of materials in the Wannier basis and employs a tailored fermionic encoding that preserves locality. We analyse the circuit costs of this approach and present a compiler that transforms density functional theory data into quantum circuit instructions -- connecting the physics of the material to the simulation circuit. The compiler automatically optimises circuits at multiple levels, from the base gate level to optimisations derived from the physics of the specific target material. We present numerical results for materials spanning a wide structural and technological range. Our results demonstrate a reduction of many orders of magnitude in circuit depth over standard prior methods that do not consider the structure of the Hamiltonian. For example our results improve resource requirements for Strontium Vanadate (SrVO$_3$) from 864 to 180 qubits for a $3\times3\times3$ lattice, and the circuit depth of a single Trotter or variational layer from $7.5\times 10^8$ to depth $884$. Although this is still beyond current hardware, our results show that materials simulation may be feasible on quantum computers without necessarily requiring scalable, fault-tolerant quantum computers, provided quantum algorithm design incorporates understanding of the materials and applications.

==> Algorithms_graveyard.tex <==
\section{VQE and TDS algorithms}\label{sec:VQE_alg}

In this section we will find bounds on the complexity of implementing the variational quantum eigensolver~\cite{peruzzo14,bharti2021noisy} (VQE) and time-dynamics simulation (TDS) algorithms for materials Hamiltonians. We begin by reviewing these algorithms before describing the details of how we implement and cost them for the systems of interest to us.

VQE is a method which aims to produce the ground state of a quantum Hamiltonian $H$ via optimising over trial quantum circuits picked from some family (``ansatz'') chosen based on advance knowledge that it may be able to represent the ground state effectively, and/or may be efficiently implementable on quantum hardware. Circuits from the ansatz have parameters which are optimised using a classical optimisation routine. This routine aims to minimise the energy with respect to $H$ of the state produced by the quantum circuit. By the variational principle, if the ground state can be represented within the ansatz and is unique, minimising the energy will find it. In practice, the optimisation routine may find a local minimum rather than the global minimum. Once an approximation to the ground state has been produced, measurements can be performed to determine properties of interest.

Here we will use the Hamiltonian variational ansatz~\cite{wecker15} within the VQE framework. This ansatz can be used to find the ground state of a Hamiltonian $H$ such that $H = \sum_{k\ge 0} H_k$, for some decomposition where we have an efficient quantum circuit for preparing the ground state of $H_0$, and the time-evolution operations $e^{i t H_k}$ can be implemented efficiently for all $k$ and arbitrary times $t$. (For example, $H_k$ may act non-trivially on only a small number of qubits.) Then we perform the following steps:
%
\begin{enumerate}
    \item Prepare the ground state of $H_0$.
    \item For each of $l$ layers, implement the operation
    %
    \[ \prod_k e^{it_{lk} H_k} \]
    %
    for some parameters $t_{lk}$, to produce a state $\ket{\psi}$. Note that we will allow the ordering of the product to be arbitrary below, which can allow for more efficient algorithms.
%    \item Measure the energy of $\ket{\psi}$ with respect to $H$.
%    \item Optimise over the parameters $t_{lk}$ to find the ground state (or a good approximation).
\end{enumerate}
%
Here we will compute the complexity of step 1, and of one layer of step 2. The terms $H_k$ will correspond to the terms in equations \eqref{eq:bandbasis} and \eqref{eq:wannierbasis} \am{I guess this isn't quite right, as those equations aren't in terms of Majoranas? Will we have equations of this form?}, depending on whether we use the band or Wannier basis. In either case, all terms correspond to quadratic or quartic Majorana operators. We will also determine the number of measurements required to measure the energy of $\ket{\psi}$ with respect to the materials Hamiltonian. To gain a full understanding of the complexity of VQE, it is also necessary to understand how many layers are required, and how efficient the optimisation process is, which we will not consider here; see~\cite{cade20,mineh21} for detailed numerical analyses of these points in the case of the Fermi-Hubbard model.

By contrast to VQE, the time-dynamics simulation (TDS) approach corresponds to implementing the unitary operation $e^{-itH}$ for some $t$. Simulating time-dynamics of a quantum system is theoretically more straightforward than finding a ground state (BQP-complete in the worst case, rather than QMA-complete), yet may be more challenging in practice for near-term quantum computers. If an algorithm based on Trotterisation is used, TDS is very similar to implementing step 2 of the VQE algorithm. However, note that we have assumed in VQE that the time-evolution steps for each $H_k$ can occur in arbitrary order, whereas we may want to fix a particular order for TDS. \am{Add further details and references about TDS?}

\subsection{Complexity model and low-level calculations}
\label{sec:prelims}

We will use a simple model where all-to-all interactions are allowed, arbitrary 2-qubit gates are cost 1 each, and 1-qubit gates are free. We will aim to minimise the overall circuit depth. For the cost calculations, we will need to determine the cost of implementing time-evolution for the quadratic and quartic terms, and the cost of fermionic swap operations.

\textbf{Time-evolution.} Whichever fermionic encoding is used, each term will ultimately be represented on the quantum computer as a string of Pauli operators. As 1-qubit gates are free and all Pauli operators are equivalent up to unitary conjugation, implementing a term reduces to implementing the operation $e^{i\theta Z \dots Z }$, acting on $k$ qubits, for arbitrary $\theta$. This can be done in depth $2\lceil \log_2 k \rceil - 1$ via a circuit which uses a binary tree of CNOT operations to put the parity of the input state in the last qubit; performs a Z rotation on that qubit; and then performs the CNOT operations in reverse to uncompute the parity. We save depth 1 by combining the last two CNOTs and the Z rotation in one 2-qubit gate. See Figure \ref{fig:paritycircuit} for an example for the case $k=4$.

Note that we may have multiple commuting terms acting on the same qubits, which can lead to efficiency savings by implementing time-evolution according to these simultaneously. However, we do not consider this in our calculations below.

\begin{figure}[t]
    \centering
    \includegraphics{Figs_algorithms/paritycircuit.pdf}
    \caption{The quantum circuit for implementing $e^{i \theta Z^{\otimes k}}$ in the case $k=4$. The three middle gates can be combined into one 2-qubit operation, given total cost (2-qubit gate depth) 3 in our model.}
    \label{fig:paritycircuit}
\end{figure}

\textbf{Fermionic swaps.} In the JW transform, fermionic swaps across adjacent modes are 2-qubit gates with cost 1. In the compact encoding, across most pairs of adjacent modes, the same holds. The exception is fermionic swaps across the split between sites, where an ancilla qubit is involved.

Here we can get an efficient decomposition as follows. Written in terms of Paulis, a fermionic swap operation on the 3 qubits including the ancilla is of the form
%
\[ \frac{1}{2} \left(Z_1 + Z_2 + (X_1 X_2 + Y_1 Y_2)Y_A \right) \]
%
\am{I need to check the other 3 types of term, but they should be basically the same.} We can diagonalise the Y on the ancilla with a local unitary. For the remaining part, $Z_1 + Z_2$ commutes with $X_1 X_2 + Y_1 Y_2$ \jk{these anti-commute...}, so we can simultaneously diagonalise this part with a 2-qubit gate, which turns out to be a Hadamard gate acting only on the odd parity subspace. Then we are left with a unitary which turns out to be $\diag(1,1,1,-1,-1,1,-1,-1)$. This can be implemented using two controlled-Z gates (controlled on the 2nd qubit). The overall 2-qubit gate depth is then 4. %Therefore, there is a multiplicative overhead of at most 4 in the complexity of fermionic swap layers.

\textbf{Givens rotations.} In the context of fermionic quantum simulation algorithms, a Givens rotation is an operation of the form
%
\[ e^{\theta(c^\dag_i c_j - c^\dag_j c_i)} = e^{i\theta(\gamma_i \bar{\gamma}_j - \bar{\gamma}_i \gamma_j)/2}. \]
%
\am{NB: different to Joel's note on Slack.} In the JW transform, when acting on adjacent modes this is a 2-qubit operation. In the compact encoding, it is usually a 2-qubit operation, except when acting across sites, when it is an operation of the form
%
\[ e^{i\theta(\gamma_i \bar{\gamma}_j - \bar{\gamma}_i \gamma_j)/2} = e^{i\theta(X_1 Y_2 - Y_1 X_2)Y_A} \]
%
\am{The sign and scaling might be wrong, but this shouldn't change anything.} By a similar argument to the fermionic swap operation (also see Appendix A of the Fermi-Hubbard VQE paper), this 3-qubit operation can be implemented in 2-qubit gate depth 4.


%-------------------------------------------------------

\subsection{Implementing time-evolution}

For both the VQE and TDS algorithms, we need to implement time-evolution according to the quadratic part and the quartic part of the materials Hamiltonians $H_B$, $H_W$.
%Here we will obtain a worst-case bound by assuming that all quadratic and quartic terms are present.
To do this efficiently, we will use a protocol  based on fermionic swap networks~\cite{kivlichan18}. These networks use layers of fermionic swap gates to rearrange the fermionic ordering and to enable interactions to be implemented efficiently -- for example, by moving modes to be adjacent in the JW transform. \am{more details...?} Theoretical constructions of fermionic swap networks are known which implement all quadratic~\cite{kivlichan18} or quartic (Microsoft patent?) interactions efficiently. However, here we will want to apply this idea to specific materials Hamiltonians that do not include all terms. We are therefore led to an algorithmic approach to produce an efficient swap network protocol for a given Hamiltonian.

We consider protocols that alternate layers of the following form:
%
\begin{enumerate}
    \item Fermionic swap gates that can be performed in depth 1 (i.e.\ involving a sequence of pairs of adjacent modes). \am{not depth 1 in the compact encoding, need to check}
    \item All quartic terms that correspond to pairs of adjacent modes (i.e.\ involving modes $i,i+1$, $j,j+1$ for some $i$ and $j$). These are the ones that can be implemented efficiently given the current ordering of modes, and assuming all-to-all connectivity.
    \am{this is a ``greedy'' protocol -- we could also implement just one layer of quartic interactions, should check if this is more efficient}
\end{enumerate}
%
The aim is then to find a protocol using a small number of layers (corresponding to a good choice of positions for fermionic swap gates), as well as implementing the quartic interaction part of each layer efficiently. We can achieve both of these using a computational technique.

To find a good sequence of fermionic swap gates, we use a greedy protocol. At each layer, we look at the set of quartic interactions $T$ which have not yet been implemented, and define a distance function which measures the difficulty of implementing these interactions. Here we focus on distance functions of the form
%
\[ D = \sum_T d(T)^\alpha, \]
%
where $\alpha \in R$ and $d(T)$ is a distance measure for a term, which should be related to the number of swaps required to bring the interaction $T$ into adjacent form. Assuming that $T$ acts on modes $i<j<k<l$,  we use $d(T) = (j-i+1) + (l-k+1)$. Empirically, we find that choosing $\alpha = 0.5$ seems to produce good results. \am{This should be replaced with what actually happens in the code, in terms of the interaction graph...}

We consider swapping each possible adjacent pair of modes ($i$, $i+1$), and compute the $D$ function for each choice. If there exists a pair whose resulting $D$ function is reduced, we then swap the pair which minimises $D$ and mark this pair as used. We repeat this process until all modes have been used, or there is no choice of modes to swap that reduces $D$. A potential issue with this approach is that even in the first step, there may be no choice of pairs to swap that reduces $D$. We can handle this by adding a fallback step where a swap operation is chosen that at least reduces $d(T)$ for some term $T$.

To implement all quartic interactions efficiently, we express this problem in terms of graph colouring. We define a graph whose vertices are quartic terms that should be implemented in the current layer, and where two vertices are connected if the corresponding terms can be implemented simultaneously. Here we take the simple view that two terms can be implemented simultaneously if they act on disjoint sets of modes. Then the minimal number of colours required to colour this graph such that no two adjacent vertices have the same colour is the same as the minimal number of layers required to implement all the terms.

As graph colouring is an NP-complete problem, we do not expect to be able to find the exact minimal number of layers for large numbers of modes. (Empirically, it seems that exact graph colouring algorithms are too slow even for $M\ge 10$ or so.) However, we can use graph colouring heuristics to find an upper bound on the minimal number of layers efficiently.

We can then express the ``quartic depth'' (the number of quartic layers) and the number of swap layers, in terms of $M$. Using this approach with the DSATUR graph colouring heuristic and a simple least-squares fit, we find that the quartic depth is $\approx 0.096 M^{3.24}$, and the swap depth is $\approx 0.13 M^{2.36}$.
This should be compared with the bounds from the Microsoft protocol of $4M^3/3$ fermionic swap layers, and about $M^3/6$ quartic depth. We see that the quartic depth is somewhat worse, but the swap depth is substantially better.

Translating this into a true circuit complexity will give different answers depending on whether we are using the Jordan-Wigner or compact encoding. In Jordan-Wigner, swapping any adjacent pair of modes has equal cost, and all quartic interactions have equal cost. In the compact encoding, considering two sites with $n_{\max}$ modes each, swapping pairs of modes between sites is more costly than swapping within sites, and similarly quartic interactions on modes either side of the split between sites are more costly.

We can take the compact encoding's constraints into account algorithmically by changing the distance function to not allow for implementing interactions across the split between sites, and on the other hand, increasing the cost of the swap part by the additional cost of swapping across this split. The first part can be achieved by penalising the distance of terms which are equidistant from the split by 2. The second part can be achieved by keeping track of swap layers involving a swap across the split, and changing the cost of such layers to 4. Making these changes, we get a quartic depth $\approx0.084 n^{3.28}$, and a swap depth $\approx 0.042 n^{2.74}$. (The second one can't be quite right, given that the swap depth can only be worse by a multiple of 4 at most.)

We are now ready to calculate the VQE layer complexities for each representation of the materials Hamiltonian.

\textbf{Bloch basis, JW transform.} The quadratic part is trivial, consisting of 1-qubit rotations with no cost. For the quartic part, if we use the protocol above we obtain a complexity of $\approx 0.096 M^{3.24}$ quartic layers, and $\approx 0.13 M^{2.36}$ swap layers. By Section \ref{sec:prelims} we assume that each quartic layer has 2-qubit gate depth 6; each swap layer has 2-qubit gate depth 1. The overall depth is then
%
\[ \approx 0.576 M^{3.24} + 0.13 M^{2.36} \approx 0.576 M^{3.24} = 0.576 (Vn_{\max})^{3.24} \]
%
per layer.

\textbf{Wannier basis, JW transform.} We can split implementing a VQE layer into two parts: swapping sites into the right position, and implementing interactions between sites. We will assume that quadratic interactions can be implemented at no additional cost, during the time that the swaps are happening. On an $L_x \times L_y$ lattice, using the same swap network as for standard Fermi-Hubbard, $2L_x$ layers of swapping adjacent sites are enough to implement all vertical interactions. Swapping two adjacent sites with $n_{\max}$ modes each can be done using $2n_{\max}-1$ layers of fermionic swaps. Finally, the interactions can be implemented using the previous technique, setting $M=2n_{\max}$. In standard Fermi-Hubbard, the vertical interactions can be implemented while horizontal swaps are taking place, at no additional depth cost. Here, however, they sometimes dominate the depth cost. Also, the horizontal interactions apparently do not come for free and need to be implemented separately at the start.

Therefore, the depth of the entire layer is
%
\[ 2 \cdot 0.576(2n_{\max})^{3.24} + L_x(2n_{\max}-1 + 0.576(2n_{\max})^{3.24}) \approx (11 + 6L_x)n_{\max}^{3.24}.
\]
Considering a square lattice, this is better than the complexity in the Bloch basis if $11+6L_x \le 0.576 L_x^3$, corresponding to $L_x \ge 4$.

\textbf{Wannier basis, compact encoding.} We can use swap networks to implement all the required interactions, for each adjacent pair of sites. As discussed above, for each pair this costs quartic depth $\approx0.084 (2n_{\max})^{3.28}$, and swap depth $\approx 0.042 (2n_{\max})^{2.74}$. By Section \ref{sec:prelims}, each quartic layer has depth 6, whereas the swap depth cost already takes into account the additional cost of the compact encoding. In 2d, we need to do this for 4 types of adjacent pair (two horizontal, two vertical). Note that the quartic interactions occurring only within each site are handled as part of the interactions between sites. Then the depth of the entire layer is
%
\[ \approx 4 \cdot 6 \cdot 0.084 (2n_{\max})^{3.28} \approx 20 n_{\max}^{3.28}. \]
%
This is lower than the cost using the JW encoding, except if $n_{\max}$ is very much larger than $L_x$.

{\color{red}
Algorithms section graveyard

\subsection{Materials Hamiltonians}

We will consider materials Hamiltonians expressed in the band and Wannier bases, as described in the previous section and defined formally in eqns \eqref{eq:bandbasis} and \eqref{eq:wannierbasis}. For clarity, in this section we write these as $H_B$, $H_W$ respectively.

\am{Is it helpful to keep rough complexity calculations like this in here? If so, they probably need some checking, as I last looked at this a long time ago, so this may be wrong\dots}
For an $L_x \times L_y \times L_z$ cubic lattice, the site index $\mathbf{R}$ and the dual lattice indices $\mathbf{k},\mathbf{q},\mathbf{k'}$ can take $V = L_x L_y L_z$ values. Each $n$ is a combination of band index and spin. We expect (e.g.)\ $1 \le L_x,L_y,L_z \le 10$, $4 \le n \le 100$ to be reasonable ranges for these parameters. The number of fermionic modes is $M:=V n_{\max}$. For realistic systems, this could then be as low as 4 (one lattice site, 4 bands with spin), or as high as $10^5$ ($10\times10\times10$ lattice, $n_{\max}=100$). So:
%
\begin{itemize}
    \item $H_B$ has $V n_{\max}$ quadratic terms, and at most $V^3 n_{\max}^4$ quartic terms. As we assume that all terms act on distinct modes, the number of quartic terms is actually upper-bounded by $\binom{V n_{\max}}{3}n_{\max} \le V^3 n_{\max}^4 / 6$ (actually slightly less, as this overcounts terms where $\kk_1+\kk_2-\kk_3=\kk_1$, for example).
    \item In 2d, $H_W$ has at most $5 V n_{\max}^2$ quadratic terms, and at most $5^3 V n_{\max}^4$ quartic terms. In 3d, there are at most $7V n_{\max}^2$ quadratic terms, and at most $7^3 V n_{\max}^4$ quartic terms.
\end{itemize}
%
So we see that if $V \ll n_{\max}$, the Bloch basis representation is more efficient, whereas if $V \gg n_{\max}$, the opposite is true.
It should be possible to heavily parallelise the corresponding quantum circuits, such that the depth reduces by a factor of approximately $V n_{\max}/2$ in each case. We further expect that the quartic terms will dominate the complexity. In 2d, this would lead to overall estimates of depth $V^2 n_{\max}^3 / 3$ for the Bloch basis, and $250 n_{\max}^3$ for the Wannier basis, predicting that the Wannier basis will be superior whenever $V \ge 28$.

This further suggests circuit depth estimates to implement a VQE layer ranging from a lower bound of 22 ($V=1,n_{\max}=4$, band basis) to numbers possibly in the millions for realistic sizes (e.g.\ $V=25,n_{\max}=20$, Wannier basis). In what follows, we will calculate detailed estimates, based on the use of fermionic swap networks.

Fermionic swap networks were introduced in the context of quantum simulation in (Google paper) based on ideas previously developed in (). ...

%-------------------------------------------------------
\begin{comment}
Commented out this section as it's discussed in the previous part
\subsection{Encoding the fermionic Hamiltonian}

We consider:

\begin{enumerate}
    \item The Jordan-Wigner transformation for all fermionic modes
    \item A hybrid encoding where we use Jordan-Wigner within sites, and a variant of the compact encoding across sites.
\end{enumerate}

Within the Jordan-Wigner transform, we can further consider different approaches for implementing the required interactions efficiently. The most naive method is to implement each one directly; if the length of the Jordan-Wigner string is $k$, the quantum circuit depth required is approximately $2\lceil \log_2 k \rceil$ (recalling that we assume all-to-all connectivity). To get a rough upper bound, we can replace this with $2\lceil \log_2 M \rceil = 2\lceil \log_2 (Vn_{\max}) \rceil$. However, although not too bad in terms of gate count, this is very bad in terms of depth, as (at least if we implement this naively) we can't parallelise any of the interactions. We will instead use fermionic swap networks, which can be much more efficient.

In the Jordan-Wigner transform, we also need to choose an ordering of the qubits. In the Bloch basis, we are not assuming any special structure, so it seems that the ordering can be arbitrary. In the Wannier basis, it seems natural to put modes which are on the same site together, and then use a ``snake'' ordering on the 2d (or 3d) lattice of sites. Within a site, it probably makes sense to organise modes according to spin (spin-up first, then spin-down).

(For Fermi-Hubbard, this wasn't the case -- but there, we didn't need to worry about long Jordan-Wigner strings for the quartic interactions.)

\am{Discussion of 3d here?}
\end{comment}

\subsection{Preparing the initial state}

For both $H_B$ and $H_W$, a natural starting point is to prepare the ground state of the quadratic part of the Hamiltonian.

\textbf{Bloch basis, JW transform.}  The ground state of the quadratic part is a computational basis state, so this is trivial.

\textbf{Wannier basis, JW transform.} We can use the algorithm of Jiang et al, ``Quantum algorithms to simulate many-body physics of correlated fermions'', based on Givens rotations. This achieves a depth of $M-1$ and a 2-qubit gate complexity of at most $M^2/4$, depending on the occupation number -- the case $M^2/4$ corresponds to half-filling.

This is likely to be close to tight, given that this encompasses the special case of the Fermi-Hubbard model.

\textbf{Wannier basis, compact encoding.} We can also use the approach of Jiang et al to prepare the initial state with this encoding. A Givens rotation is a unitary operation of the form $e^{i\theta Y}$ acting on two fermionic modes. The only pairs required to be acted on are consecutive in an arbitrary ordering of the modes. If the modes are on the same site, this requires a 2-qubit gate. However, if they are on different sites, the operation acts on 3 qubits.

The algorithm of Jiang et al acts on (at most) all consecutive modes at each step in an even-odd pattern. If we act on an even number of modes in total (as will always be the case if we consider spin) then at every other step, we only have 2-qubit gates. By Section \ref{sec:prelims}, the depth of the step involving 3-qubit gates is 4. Therefore, the overall depth is at most $4 \lceil (M-1)/2 \rceil + \lfloor (M-1)/2 \rfloor \approx 2.5M$.


\textbf{Time-evolution.} The most complicated terms to consider are quartic terms involving 4 distinct modes, which (assuming time-reversal symmetry) are of the form
%
\[ \gamma_1 \gamma_2 \gamma_3 \gamma_4 + \bar{\gamma}_1\bar{\gamma}_2\bar{\gamma}_3\bar{\gamma}_4 - 2\gamma_1 \gamma_2 \bar{\gamma}_3 \bar{\gamma}_4 + 4 \bar{\gamma}_1 \gamma_2 \gamma_3 \bar{\gamma}_4, \]
%
corresponding to the real part of the Hamiltonian from... \am{will be included, was in Joel's notes}. In the Jordan-Wigner transform this becomes
%
\[ XXXX + YYYY - 2XXYY + 4YXXY \]
%
\am{should there also be XYYX terms?} if we restrict to considering pairs of adjacent modes only (i.e.\ $(i,i+1)$, $(j,j+1)$). These 4 terms commute. Observe that $XX$ and $YY$ can be simultaneously diagonalised by a 2-qubit transformation, corresponding to switching to the Bell basis, giving $IZ$ and $ZI$. Performing this two-qubit gate on qubits $1,2$ and $3,4$ simultaneously, the first three terms in the Hamiltonian are transformed to
%
\[ IZIZ + ZIZI - 2IZZI. \]
%
The required 2-qubit rotations can then be performed in depth 2. The remaining term $4YXXY$ can be handled separately by a similar transformation on pairs of qubits. The resulting circuit then has 2-qubit gate depth 6 (depth 1 to switch into the Bell basis; depth 2 to time-evolve; depth 1 to switch into the XY/YX basis; depth 1 to time-evolve; and depth 1 to switch back into the computational basis). \am{Quantum circuit diagrams should be included for these.}

If the imaginary part is required (which does not commute with the real part), a similar approach can be applied. Transform
%
\[ YXXX - XYYY \mapsto XXXX - YYYY \mapsto IZIZ - ZIZI, \]
%
where the first transformation requires only local unitaries and the second uses a transformation into the Bell basis. Then the two time-evolution operations can be performed in parallel; we end up with 2-qubit depth 3 in total. In the compact encoding, the situation is the same, unless we need to perform quartic terms across sites. Here we will enforce that this never happens.

\textbf{Terms on three distinct modes.} We will also need to consider terms of the form $c_1^\dag c_1 c_2^\dag c_3$. By Hermiticity, we can actually restrict to considering terms of the form $c_1^\dag c_1 (c_2^\dag c_3 + c_3^\dag c_2)$. In the Jordan-Wigner transform, this corresponds to the operator $(I+Z)(XX+YY)$. Transforming the last 2 qubits to the Bell basis, we obtain $IIZ + IZI + ZIZ + ZZI$; time-evolution according to this can be achieved with 2-qubit gate depth 2, and some 1-qubit gates. The overall 2-qubit gate depth is 4.

}

%-------------------------------------------------------

\subsection{Measurements}

We assume for now that we want to measure all quadratic and quartic terms, expressed in terms of Majorana operators. In the Jordan-Wigner picture, the quadratic case corresponds to strings of the form $XZZ\dots ZY$, where the first operator may begin or end with either $X$ or $Y$, and the quartic case is products of two such strings on disjoint indices. We further assume that we only need to measure quartic terms containing an even number of $X$'s \am{Corresponds to the materials Hamiltonian having no imaginary part?}. We can then categorise quadratic or quartic terms as either XX/YY-type or XY/YX-type. The type of a quadratic term is its endpoints. The type of a quartic term is the type of both of its quadratic terms (by the constraint on having an even number of $X$'s, both terms must be of the same type).

A naive measurement strategy would measure each term in sequence, using $\Theta(M^4)$ measurements. Our goal here will be to do better by measuring multiple terms at a time. Minimising the number of rounds may not always give the strategy requiring the minimal number of measurements to achieve a certain level of accuracy, as this also depends on the variance of each measurement; however, this approach is a reasonable starting point. We also look for the measurements to be implemented using straightforward (ideally constant-depth) quantum circuits. To this end, we consider three types of measurement strategies:

\begin{itemize}
    \item \textbf{(DIS)} Measuring terms on disjoint sets of qubits simultaneously. This family of measurement strategies is easy to implement by measuring each qubit in the correct X/Y/Z basis, so requires only additional single-qubit gates. In the literature, this concept is often called qubitwise commutativity \am{cite...}.
    
    \item \textbf{(NC)} Measuring a family of \emph{non-crossing} terms simultaneously. We say that a set of terms (Majoranas) is non-crossing if there is no pair $(i,j)$, $(k,l)$ corresponding to an interaction between mode $i$ and $j$, and between mode $k$ and $l$, such that $i < k < j < l$. A set of terms of XX/YY or XY/YX type in the JW transformation can be measured simultaneously in a simple way if they are non-crossing. This is because $XX$, $YY$ and $ZZ$ commute and hence can be measured simultaneously (by a simple local transformation); the same is true for the set $\{XY,YX,ZZ\}$. So if all endpoints of all hopping terms are either both contained within the $Z$-string of another hopping term, or avoid that hopping term completely, we can measure the terms simultaneously.
    
    An NC protocol corresponds to a non-crossing matching on the complete graph with $M$ vertices, where we apply a 2-qubit unitary to the endpoints of each edge in the matching, and then measure in the computational basis. Such a protocol allows us to measure all the corresponding quadratic terms (and hence their products) simultaneously.
    
    \am{Discuss Hamamura and Imamichi, 2020}.
    
    \item \textbf{(COM)} Measuring a family of commuting operators simultaneously. This is the most general approach we will consider, so will require correspondingly fewer measurement rounds. However, the quantum circuits required to simultaneously diagonalise a set of measurement operators may be relatively difficult to implement (requiring depth $\Theta(M)$). 
\end{itemize}

We will obtain analytical upper and lower bounds for each type of strategy, before moving on to computational upper bounds.

\subsubsection{Analytical upper bounds}

\textbf{(DIS)} \am{Fill in}

\textbf{(NC)} We describe an explicit protocol that uses $M^2(M-1)/2$ measurement rounds to measure all XX/YY-type quartic terms (and similarly XY/YX-type quartic terms), leading to a complexity of $M^2(M-1)$ measurement rounds in the protocol. We first claim that an arbitrary set of quadratic terms on $M$ modes of a given type can be measured in at most $M$ rounds. See Figure \ref{fig:quad_measurements} for how this can be done. Then, to measure all quartic terms, we fix the first quadratic term and apply the quadratic-term protocol to the others. The total complexity is $M^2(M-1)/2$.

\textbf{(COM)} An analytical $O(M^3)$ upper bound was shown in~\cite{gokhale20}. \am{Fill in / cite other work}

\begin{figure}
    \centering
    \includegraphics[width=5cm]{Figs_algorithms/rainbow2.png}\hspace{1cm}
    \includegraphics[width=5cm]{Figs_algorithms/rainbow1.png}
    \caption{How to implement measurements of all quadratic terms in $M$ rounds, for $M=5,6$. The modes are divided into two rainbows, and the size of the left-hand rainbow grows by 1 in each round.}
    \label{fig:quad_measurements}
\end{figure}

\subsubsection{Analytical lower bounds}

\textbf{(DIS)} We produce a set of $\Omega(M^4)$ quartic terms, each pair of which acts on an overlapping set of qubits, as products of pairs of quadratic terms. Assume for simplicity that $M$ is a multiple of 4. The first set of quadratic terms is
%
\[ T_1 = \{\eta_{M/4-i} \zeta_{M/4+j+1}: i,j \in \{0,\dots,M/4-1\}, \eta,\zeta \in \{\gamma,\bar{\gamma}\} \} \]
%
and the second is
%
\[ T_2 = \{\eta_{3M/4-i} \zeta_{3M/4+j+1}: i,j \in \{0,\dots,M/4-1\}, \eta,\zeta \in \{\gamma,\bar{\gamma}\} \}. \]
%
Each pair of terms in $T_1$ acts on modes $M/4$, $M/4+1$, and similarly each pair of terms in $T_2$ acts on modes $3M/4$, $3M/4+1$. Therefore each pair of products of terms from $T_1$, $T_2$ overlaps and cannot be measured simultaneously. $|T_1| = |T_2| = M^2/4$, so we obtain a lower bound of $M^4/16$ measurements.

\textbf{(NC)} Each rainbow diagram introduced above can be mapped univocally to a Motzkin path. A Motzkin path is a lattice path in the plane integer lattice
$\mathbb{Z}\times\mathbb{Z}$ consisting of up steps $(1, 1)$, down steps $(1, -1)$ and horizontal steps $(1,0)$ which never passes below the
x-axis. The map from a rainbow diagram is simple. Reading the diagram from left to right, if at site $j$ we encounter an arc going up (down) we take a step $(1,1)$ ($(1,-1)$) from $j$ to $j+1$, (see Fig. \ref{fig:map_motzkin} for an example). The number of Motzkin paths with the $n_i$ steps up at height $i$ and $m_i$ horizontal steps at height $i$ is \cite{Oste2015}
\begin{equation}
 \rho(\mathbf{n},\mathbf{m})={n_1+m_0\choose m_0}\prod_{i\geq 1}{n_i+n_{i+1}+m_i-1\choose m_i}\prod_{i\geq 1}{n_i+n_{i+1}-1\choose n_{i+1}},
\end{equation}
where $\mathbf{n}=(n_1,n_2,\dots)$ and $\mathbf{m}=(m_0,m_1,\dots)$
\begin{figure}
    \centering
    \includegraphics[width=12cm]{Figs_algorithms/map_motzkin.png}
    \caption{Map from rainbows to Motzkin paths}
    \label{fig:map_motzkin}
\end{figure}


We can bound the number of measurement needed by counting the most extended Motzkin paths that correspond to four fermion terms as they cannot be measured in parallel. These are given in Fig. \ref{fig:Motzkin_paths_4_fer}.

By this account, adding all the contributions we have $ \mbox{\# measurements} \geq \frac{3}{2}M^2-\frac{13}{2}M+1$.
We can make this bound tighter by including Motzkin paths with smaller base, but with care of not counting configurations that can be measured in parallel with any of the previous ones. The paths of diagram (\ref{fig:Motzkin_path2}) cannot be measured in parallel with any of the previous ones so the total number of extra measuments needed is ${{M-4} \choose 2}$ per path type, which added to the original tally gives
\begin{equation}
 \mbox{\# measurements} \geq \frac{5}{2}M^2-\frac{27}{2}M+13.
\end{equation}
Further optimizations of the lower bound are possible including extra paths.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figs_algorithms/Motzkin_paths_4_fer.png}
    \caption{Extended four fermion configurations that cannot be measured in parallel due to overlapping strings of Pauli Z in the Jordan-Wigner encoding.}
    \label{fig:Motzkin_paths_4_fer}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figs_algorithms/Motzkin_path2.png}
    \caption{Extra paths that can be included in the tally.}
    \label{fig:Motzkin_path2}
\end{figure}

\textbf{(COM)} Here we can prove a lower bound of $\Omega(M^2)$ measurements. For this it is sufficient to find a set of $\Omega(M^2)$ quartic terms, each pair of which anticommutes, as no such pair can be measured in the same round. We construct such a set of terms as a product of two quadratic terms $t_1$, $t_2$ picked from sets $T_1$, $T_2$, such that each pair of terms in $T_1$ anticommutes, and each pair of terms in $T_2$ commutes. We choose
%
\[ T_1 = \{\gamma_1 \gamma_i^\dag : i \in \{2,\dots,M/2\} \} \cup \{\gamma_1 \bar{\gamma}_i^\dag : i \in \{2,\dots,M/2\} \} \]
%
and
%
\[ T_2 = \{ \eta_{2i+1} \zeta^\dag_{2i+2} : i \in \{M/4,\dots,M/2-1\}, \eta,\zeta \in \{\gamma,\bar{\gamma} \} \}, \]
%
assuming for simplicity that $M$ is a multiple of 4. Then $|T_1| = M - 2$, $|T_2| = M$, so we obtain a lower bound of $M(M-2)$ measurements.

\subsubsection{Computational upper bounds from graph colouring}

We can express the problem of finding the minimal number of measurement rounds for a given strategy as a graph colouring problem. Each vertex corresponds to a quartic term, and two vertices are connected by an edge when they are incompatible with respect to one of the above strategies (i.e.\ act on the same qubit, cross, or anticommute). Compatible terms can be measured in the same round. The number of colours required then corresponds to the number of measurement rounds.

We solved the graph colouring problem using the DSATUR heuristic (and others) implemented in the NetworkX Python package. Using an exact graph colouring tool was too slow except for the smallest sizes ($M\le 10$). Using the heuristic tool suggests that the complexity scaling for each of the strategies is approximately $0.016 M^{3.91}$ for DIS, $0.074 M^{2.93}$ for NC, and $0.059 M^{2.73}$ for COM, based on fitting to instances on $M\le 28$ (or less). Further experiments should be performed to determine the complexity scaling more accurately by considering larger $M$. Henceforth we restrict to the NC strategy, as it provides a good balance between number of measurement rounds and complexity (saving a factor of almost $M$ compared with DIS, while needing only one more layer of 2-qubit gates).

\textbf{Bloch basis, JW transform.} By the above analysis for the NC strategy, we immediately obtain a complexity of $\approx 0.074 (Vn_{\max})^{2.93}$.

\textbf{Wannier basis, JW transform (2d).} It is natural to split the terms up into 4 parts, corresponding to the 4 types of edges in a 2d square lattice. We treat each of the edges as an individual system on $2n_{\max}$ modes and measure each one in turn -- note that there could be a lot of other Z operators, but these don't matter, as they commute with all sites in between. Terms local to each site are already encompassed by these edges, so don't need to be measured again. The overall complexity using the NC strategy is then $\approx 4\cdot 0.074 (2n_{\max})^{2.93} \le 3n_{\max}^{2.93}$ measurement rounds, a substantial saving of $O(V^3)$ compared with the Bloch basis.

\textbf{Wannier basis, compact encoding.} The idea is very similar to the JW transform. The only difference is that some Majoranas that we need to measure will be a little more complicated, as we have the ancilla qubit in the way. The overall complexity should be the same \am{check!} -- at most $3n_{\max}^{2.93}$.

%-------------------------------------------------------

\subsection{Summary of complexities}

\am{This should include 2d and 3d}

\begin{table}[b]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
         Method & Initialisation & VQE layer & Measurement & Total circuit depth \\
        \hline Bloch + JW & 0 & $0.576L^{6.48} n_{\max}^{3.24}$ & $O(L^6 n_{\max}^3)$ & $0.576pL^{6.48} n_{\max}^{3.24}$ \\
        Wannier + JW & $L^2 n_{\max}-1$ & $6L n_{\max}^{3.24}$ & $O(n_{\max}^{2.93})$ & $6pL n_{\max}^{3.24}$ \\
        Wannier + compact & $2.5 L^2 n_{\max}$ & $20 n_{\max}^{3.28}$ & $O(n_{\max}^{2.93})$ & $20 p n_{\max}^{3.28}$ \\
        \hline
    \end{tabular}
    \caption{Complexity of implementing $p$ VQE layers, in the special case of an $L \times L$ 2d lattice. All complexities are approximate.}
    \label{tab:my_label}
\end{table}


==> Figs_Results/full_approx_just_srvo3.tex <==
\begin{tabular}{lllrrrr}
\toprule
         &     &         &  Swaps &  Onsite/NN &  NNN+ &  Total \\
Material & Qubits & Algorithm &        &            &       &        \\
\midrule
\multirow{4}{*}{SrVO$_3$} & \multirow{4}{*}{180} & TDS &    336 &         59 &   744 &   1139 \\
         &     & TDS$^*$ &      0 &        545 &   744 &   1289 \\
         &     & VQE &    336 &         59 &   500 &    895 \\
         &     & VQE$^*$ &      0 &        545 &   500 &   1045 \\
\bottomrule
\end{tabular}


==> Figs_Results/full_approx_summary_table.tex <==
\begin{tabular}{lllrrr}
\toprule
                   &      &         &  Swaps &  Onsite/NN &  Total \\
Material & Qubits & Algorithm &        &            &        \\
\midrule
\multirow{4}{*}{GaAs} & \multirow{4}{*}{1120} & TDS &    444 &         90 &    534 \\
                   &      & TDS$^*$ &      0 &       1147 &   1147 \\
                   &      & VQE &    444 &         90 &    534 \\
                   &      & VQE$^*$ &      0 &       1129 &   1129 \\
\cline{1-6}
\cline{2-6}
\multirow{4}{*}{H$_3$S} & \multirow{4}{*}{1870} & TDS &    864 &         96 &    960 \\
                   &      & TDS$^*$ &      0 &       7045 &   7045 \\
                   &      & VQE &    864 &         96 &    960 \\
                   &      & VQE$^*$ &      0 &       7027 &   7027 \\
\cline{1-6}
\cline{2-6}
\multirow{4}{*}{Li$_2$CuO$_2$} & \multirow{4}{*}{1024} & TDS &   1276 &        166 &   1442 \\
                   &      & TDS$^*$ &      0 &       4024 &   4024 \\
                   &      & VQE &   1276 &        166 &   1442 \\
                   &      & VQE$^*$ &      0 &       3886 &   3886 \\
\cline{1-6}
\cline{2-6}
\multirow{4}{*}{Si} & \multirow{4}{*}{1120} & TDS &    444 &        102 &    546 \\
                   &      & TDS$^*$ &      0 &       1821 &   1821 \\
                   &      & VQE &    444 &        102 &    546 \\
                   &      & VQE$^*$ &      0 &       1791 &   1791 \\
\cline{1-6}
\cline{2-6}
\multirow{4}{*}{SrVO$_3$} & \multirow{4}{*}{180} & TDS &    336 &         59 &    395 \\
                   &      & TDS$^*$ &      0 &        545 &    545 \\
                   &      & VQE &    336 &         59 &    395 \\
                   &      & VQE$^*$ &      0 &        545 &    545 \\
\cline{1-6}
\cline{2-6}
\multirow{4}{*}{SrVO$_3$$^\dagger$} & \multirow{4}{*}{3120} & TDS &   1480 &        180 &   1660 \\
                   &      & TDS$^*$ &      0 &       9619 &   9619 \\
                   &      & VQE &   1480 &        180 &   1660 \\
                   &      & VQE$^*$ &      0 &       9572 &   9572 \\
\bottomrule
\end{tabular}


==> Figs_Results/materials_results/alt_intro_table.tex <==
\begin{tabular}{lllrrr}
\toprule
              &                                                       &          &  Bands &  Qubits &   Depth \\
Material & Applications & Method &        &         &         \\
\midrule
\multirow{2}{*}{SrVO$_3$} & \multirow{2}{*}{Solar cells \cite{srvo3_solar_cell}, batteries \cite{svo_anode, svo_cathode}} & This work &      3 &     180 & 7.3E+02 \\
              &                                                       & Previous &     22 &    1188 & 1.3E+09 \\
\cline{1-6}
\cline{2-6}
\multirow{2}{*}{GaAs} & \multirow{2}{*}{\makecell{Semiconductors \cite{GaAs_semi}, transistors \cite{shur1987gaas}, \\solar cells\cite{Jun2013}, spintronics \cite{Okamoto2014}}} & This work &      4 &    1120 & 4.9E+03 \\
              &                                                       & Previous &     36 &    9000 & 1.2E+11 \\
\cline{1-6}
\cline{2-6}
\multirow{2}{*}{H$_3$S} & \multirow{2}{*}{Superconductors \cite{Drozdov2015}} & This work &      7 &    1870 & 2.8E+04 \\
              &                                                       & Previous &     12 &    3000 & 4.4E+09 \\
\cline{1-6}
\cline{2-6}
\multirow{2}{*}{Si} & \multirow{2}{*}{Semiconductors \cite{si_semi}, solar cells \cite{si_sc}} & This work &      4 &    1120 & 5.2E+03 \\
              &                                                       & Previous &      0 &       0 & 0.0E+00 \\
\cline{1-6}
\cline{2-6}
\multirow{2}{*}{Li$_2$CuO$_2$} & \multirow{2}{*}{High-capacity battery cathode \cite{Jing2017Li2CuO2}} & This work &     11 &    1024 & 8.0E+03 \\
              &                                                       & Previous &     26 &    6500 & 4.4E+10 \\
\bottomrule
\end{tabular}


==> Figs_Results/materials_results/apdx_data_w_n_terms.tex <==
\begin{tabular}{lllllllrr}
\toprule
         &   &                       &     &     &           &           &  Interactions &  Depth \\
Material & Bands & Dimension & Modes & Qubits & Algorithm & Terms &               &        \\
\midrule
\multirow{8}{*}{GaAs} & \multirow{8}{*}{4} & \multirow{8}{*}{$5 \times 5 \times 5$} & \multirow{8}{*}{1000} & \multirow{8}{*}{1120} & \multirow{2}{*}{TDS} & NNN+ &         22080 &   9305 \\
         &   &                       &     &     &           & Onsite/NN &         27500 &    664 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{TDS$^{*}$} & NNN+ &         22080 &   9305 \\
         &   &                       &     &     &           & Onsite/NN &         27500 &   1090 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{VQE} & NNN+ &         22080 &   7191 \\
         &   &                       &     &     &           & Onsite/NN &         27500 &    662 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{VQE$^{*}$} & NNN+ &         22080 &   7191 \\
         &   &                       &     &     &           & Onsite/NN &         27500 &   1072 \\
\cline{1-9}
\cline{2-9}
\cline{3-9}
\cline{4-9}
\cline{5-9}
\cline{6-9}
\multirow{8}{*}{H$_3$S} & \multirow{8}{*}{7} & \multirow{8}{*}{$5 \times 5 \times 5$} & \multirow{8}{*}{1750} & \multirow{8}{*}{1870} & \multirow{2}{*}{TDS} & NNN+ &         46376 &  38228 \\
         &   &                       &     &     &           & Onsite/NN &         52925 &   1217 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{TDS$^{*}$} & NNN+ &         46376 &  38228 \\
         &   &                       &     &     &           & Onsite/NN &         52925 &   7024 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{VQE} & NNN+ &         46376 &  36126 \\
         &   &                       &     &     &           & Onsite/NN &         52925 &   1214 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{VQE$^{*}$} & NNN+ &         46376 &  36126 \\
         &   &                       &     &     &           & Onsite/NN &         52925 &   7000 \\
\cline{1-9}
\cline{2-9}
\cline{3-9}
\cline{4-9}
\cline{5-9}
\cline{6-9}
\multirow{8}{*}{Li$_2$CuO$_2$} & \multirow{8}{*}{11} & \multirow{8}{*}{$5 \times 3 \times 3$} & \multirow{8}{*}{990} & \multirow{8}{*}{1024} & \multirow{2}{*}{TDS} & NNN+ &          3344 &   6885 \\
         &   &                       &     &     &           & Onsite/NN &         13953 &   1675 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{TDS$^{*}$} & NNN+ &          3344 &   6885 \\
         &   &                       &     &     &           & Onsite/NN &         13953 &   3385 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{VQE} & NNN+ &          3344 &   6710 \\
         &   &                       &     &     &           & Onsite/NN &         13953 &   1667 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{VQE$^{*}$} & NNN+ &          3344 &   6710 \\
         &   &                       &     &     &           & Onsite/NN &         13953 &   3341 \\
\cline{1-9}
\cline{2-9}
\cline{3-9}
\cline{4-9}
\cline{5-9}
\cline{6-9}
\multirow{8}{*}{Si} & \multirow{8}{*}{4} & \multirow{8}{*}{$5 \times 5 \times 5$} & \multirow{8}{*}{1000} & \multirow{8}{*}{1120} & \multirow{2}{*}{TDS} & NNN+ &         22880 &   8904 \\
         &   &                       &     &     &           & Onsite/NN &         30300 &    706 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{TDS$^{*}$} & NNN+ &         22880 &   8904 \\
         &   &                       &     &     &           & Onsite/NN &         30300 &   1746 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{VQE} & NNN+ &         22880 &   7857 \\
         &   &                       &     &     &           & Onsite/NN &         30300 &    704 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{VQE$^{*}$} & NNN+ &         22880 &   7857 \\
         &   &                       &     &     &           & Onsite/NN &         30300 &   1733 \\
\cline{1-9}
\cline{2-9}
\cline{3-9}
\cline{4-9}
\cline{5-9}
\cline{6-9}
\multirow{8}{*}{SrVO$_3$} & \multirow{8}{*}{3} & \multirow{8}{*}{$3 \times 3 \times 3$} & \multirow{8}{*}{162} & \multirow{8}{*}{180} & \multirow{2}{*}{TDS} & NNN+ &           288 &    700 \\
         &   &                       &     &     &           & Onsite/NN &          3159 &    408 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{TDS$^{*}$} & NNN+ &           288 &    700 \\
         &   &                       &     &     &           & Onsite/NN &          3159 &    552 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{VQE} & NNN+ &           288 &    476 \\
         &   &                       &     &     &           & Onsite/NN &          3159 &    408 \\
\cline{6-9}
         &   &                       &     &     & \multirow{2}{*}{VQE$^{*}$} & NNN+ &           288 &    476 \\
         &   &                       &     &     &           & Onsite/NN &          3159 &    555 \\
\bottomrule
\end{tabular}


==> Figs_Results/materials_results/appdx_all_data_w_bug.tex <==
% This version appeared in the arxiv paper but includes a small bug which should be fixed in later versions

\begin{tabular}{lllllllrr}
\toprule
Material & Bands & Dimension & Modes & Qubits & Algorithm & Dataset & Interactions &  Depth \\
\midrule
\multirow{12}{*}{GaAs} & \multirow{12}{*}{4} & \multirow{12}{*}{5x5x5} & \multirow{12}{*}{1000} & \multirow{12}{*}{1120} & \multirow{3}{*}{TDS} & Onsite/NN &         27900 &    534 \\
         &    &       &      &      &           & NNN+ &         22080 &   6033 \\
         &    &       &      &      &           & Total &         49980 &   6567 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{TDS$^{*}$} & Onsite/NN &         27900 &   1147 \\
         &    &       &      &      &           & NNN+ &         22080 &   6033 \\
         &    &       &      &      &           & Total &         49980 &   7180 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{VQE} & Onsite/NN &         27900 &    534 \\
         &    &       &      &      &           & NNN+ &         22080 &   4401 \\
         &    &       &      &      &           & Total &         49980 &   4935 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{VQE$^{*}$} & Onsite/NN &         27900 &   1129 \\
         &    &       &      &      &           & NNN+ &         22080 &   4401 \\
         &    &       &      &      &           & Total &         49980 &   5530 \\
\cline{1-9}
\cline{2-9}
\cline{3-9}
\cline{4-9}
\cline{5-9}
\cline{6-9}
\multirow{12}{*}{H$_3$S} & \multirow{12}{*}{7} & \multirow{12}{*}{5x5x5} & \multirow{12}{*}{1750} & \multirow{12}{*}{1870} & \multirow{3}{*}{TDS} & Onsite/NN &         52925 &    960 \\
         &    &       &      &      &           & NNN+ &         46376 &  30243 \\
         &    &       &      &      &           & Total &         99301 &  31203 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{TDS$^{*}$} & Onsite/NN &         52925 &   7045 \\
         &    &       &      &      &           & NNN+ &         46376 &  30243 \\
         &    &       &      &      &           & Total &         99301 &  37288 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{VQE} & Onsite/NN &         52925 &    960 \\
         &    &       &      &      &           & NNN+ &         46376 &  27284 \\
         &    &       &      &      &           & Total &         99301 &  28244 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{VQE$^{*}$} & Onsite/NN &         52925 &   7027 \\
         &    &       &      &      &           & NNN+ &         46376 &  27284 \\
         &    &       &      &      &           & Total &         99301 &  34311 \\
\cline{1-9}
\cline{2-9}
\cline{3-9}
\cline{4-9}
\cline{5-9}
\cline{6-9}
\multirow{12}{*}{Li$_2$CuO$_2$} & \multirow{12}{*}{11} & \multirow{12}{*}{5x3x3} & \multirow{12}{*}{990} & \multirow{12}{*}{1024} & \multirow{3}{*}{TDS} & Onsite/NN &         20859 &   1442 \\
         &    &       &      &      &           & NNN+ &          7760 &   6819 \\
         &    &       &      &      &           & Total &         28619 &   8261 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{TDS$^{*}$} & Onsite/NN &         20859 &   4024 \\
         &    &       &      &      &           & NNN+ &          7760 &   6819 \\
         &    &       &      &      &           & Total &         28619 &  10843 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{VQE} & Onsite/NN &         20859 &   1442 \\
         &    &       &      &      &           & NNN+ &          7760 &   6552 \\
         &    &       &      &      &           & Total &         28619 &   7994 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{VQE$^{*}$} & Onsite/NN &         20859 &   3886 \\
         &    &       &      &      &           & NNN+ &          7760 &   6552 \\
         &    &       &      &      &           & Total &         28619 &  10438 \\
\cline{1-9}
\cline{2-9}
\cline{3-9}
\cline{4-9}
\cline{5-9}
\cline{6-9}
\multirow{12}{*}{Si} & \multirow{12}{*}{4} & \multirow{12}{*}{5x5x5} & \multirow{12}{*}{1000} & \multirow{12}{*}{1120} & \multirow{3}{*}{TDS} & Onsite/NN &         30300 &    546 \\
         &    &       &      &      &           & NNN+ &         22880 &   6307 \\
         &    &       &      &      &           & Total &         53180 &   6853 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{TDS$^{*}$} & Onsite/NN &         30300 &   1821 \\
         &    &       &      &      &           & NNN+ &         22880 &   6307 \\
         &    &       &      &      &           & Total &         53180 &   8128 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{VQE} & Onsite/NN &         30300 &    546 \\
         &    &       &      &      &           & NNN+ &         22880 &   4698 \\
         &    &       &      &      &           & Total &         53180 &   5244 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{VQE$^{*}$} & Onsite/NN &         30300 &   1791 \\
         &    &       &      &      &           & NNN+ &         22880 &   4698 \\
         &    &       &      &      &           & Total &         53180 &   6489 \\
\cline{1-9}
\cline{2-9}
\cline{3-9}
\cline{4-9}
\cline{5-9}
\cline{6-9}
\multirow{12}{*}{SrVO$_3$} & \multirow{12}{*}{3} & \multirow{12}{*}{3x3x3} & \multirow{12}{*}{162} & \multirow{12}{*}{180} & \multirow{3}{*}{TDS} & Onsite/NN &          3159 &    395 \\
         &    &       &      &      &           & NNN+ &           288 &    486 \\
         &    &       &      &      &           & Total &          3447 &    881 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{TDS$^{*}$} & NNN+ &           288 &    486 \\
         &    &       &      &      &           & Onsite/NN &          3159 &    545 \\
         &    &       &      &      &           & Total &          3447 &   1031 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{VQE} & NNN+ &           288 &    336 \\
         &    &       &      &      &           & Onsite/NN &          3159 &    395 \\
         &    &       &      &      &           & Total &          3447 &    731 \\
\cline{6-9}
         &    &       &      &      & \multirow{3}{*}{VQE$^{*}$} & NNN+ &           288 &    336 \\
         &    &       &      &      &           & Onsite/NN &          3159 &    545 \\
         &    &       &      &      &           & Total &          3447 &    881 \\
\bottomrule
\end{tabular}


==> Figs_Results/materials_results/intro_results_alt.tex <==
    \begin{tabular}{|c|c|cccc|}
        \hline
        Material & some applications & method & bands & qubits & depth \\
        \hline
        SrVO$_3$  & Batteries \cite{suntivich2011design}, High T$_c$ superconductors \cite{bednorz1986} &  previous & 22 & 594 & $1.3\times 10^{9}$  \\
            & Solar cells \cite{park2015perovskite}& this work & 2 & 180 & 395\\
        \hline
        GaAs  & Semiconductors, Transistors \cite{shur1987gaas} &  previous & 36& 4500 & $1.2\times 10^{11}$  \\
            & Solar cells\cite{Jun2013}, Spintronics \cite{Okamoto2014}& this work & 5 & 1120 & 534 \\
        \hline
        H$_3$S  & High T$_c$ superconductors \cite{Drozdov2015} &  previous &12 & 1500 & $4.4\times 10^9$  \\
            & & this work & 6 & 1870 & 960\\
        \hline
        Li$_2$CuO$_2$& High-capacity battery cathode \cite{Jing2017Li2CuO2} & previous & 26 & 3250 & $4.4\times 10^{10}$  \\
            & & this work & 10& 1024 & 1442 \\
        \hline
    \end{tabular}


==> Figs_Results/materials_results/intro_table_w_bug.tex <==
% This version appeared in the arxiv paper but includes a small bug which should be fixed in later versions

\begin{tabular}{lllrrr}
\toprule
         &                                                                              &                   &  Bands &  Qubits &   Depth \\
Material & Applications & Method &        &         &         \\
\midrule
\multirow{2}{*}{GaAs} & \multirow{2}{*}{\makecell{Semiconductors \cite{GaAs_semi}, transistors \cite{shur1987gaas}, \\solar cells \cite{Jun2013}, spintronics \cite{Okamoto2014}}} & This work &      4 &    1120 & 4.9E+03 \\
         &                                                                              & Baseline estimate &     18 &    4500 & 1.2E+11 \\
\cline{1-6}
\cline{2-6}
\multirow{2}{*}{H$_3$S} & \multirow{2}{*}{Superconductors \cite{Drozdov2015}} & This work &      7 &    1870 & 2.8E+04 \\
         &                                                                              & Baseline estimate &      6 &    1500 & 4.0E+09 \\
\cline{1-6}
\cline{2-6}
\multirow{2}{*}{Li$_2$CuO$_2$} & \multirow{2}{*}{High-capacity battery cathode \cite{Jing2017Li2CuO2}} & This work &     11 &    1024 & 8.0E+03 \\
         &                                                                              & Baseline estimate &     11 &     990 & 1.1E+09 \\
\cline{1-6}
\cline{2-6}
\multirow{2}{*}{Si} & \multirow{2}{*}{Semiconductors \cite{si_semi}, solar cells \cite{si_sc}} & This work &      4 &    1120 & 5.2E+03 \\
         &                                                                              & Baseline estimate &      3 &     750 & 4.8E+08 \\
\cline{1-6}
\cline{2-6}
\multirow{2}{*}{SrVO$_3$} & \multirow{2}{*}{Solar cells \cite{srvo3_solar_cell}, batteries \cite{svo_anode, svo_cathode}} & This work &      3 &     180 & 7.3E+02 \\
         &                                                                              & Baseline estimate &     16 &     864 & 7.5E+08 \\
\bottomrule
\end{tabular}


==> Figs_Results/materials_results/srv_only.tex <==
\begin{tabular}{llrrrrr}
\toprule
         &  & \multicolumn{2}{c}{\ \ Onsite/NN} & \multicolumn{2}{c}{\ \ \ \ \ \ \  NNN+} & Total \\
         &  & Interactions & Swaps & Interactions & Swaps &  \\
 & Algorithm &              &       &              &       &       \\
\midrule
\multirow{4}{*}{SrVO$_3$} & TDS &           72 &   336 &          700 &     0 &  1108 \\
         & TDS$^{*}$ &          552 &     0 &          700 &     0 &  1252 \\
         & VQE &           72 &   336 &          476 &     0 &   884 \\
         & VQE$^{*}$ &          555 &     0 &          476 &     0 &  1031 \\
\bottomrule
\end{tabular}


==> Figs_Results/model_ham_costs_no_swaps.tex <==
\begin{tabular}{lllllrr}
\toprule
{} &      Monomial & Pauli string &    Edge &    Support &  Weight &  Cost \\
Layer &               &              &         &            &         &       \\
\midrule
0     &        (0, 5) &         XZXI &  \{0, 2\} &  \{0, 1, 2\} &       3 &     3 \\
0     &        (6, 7) &         IIIZ &     \{3\} &        \{3\} &       1 &     0 \\
1     &        (1, 4) &         YZYI &  \{0, 2\} &  \{0, 1, 2\} &       3 &     3 \\
2     &        (2, 7) &         IXZX &  \{1, 3\} &  \{1, 2, 3\} &       3 &     3 \\
2     &        (0, 1) &         ZIII &     \{0\} &        \{0\} &       1 &     0 \\
3     &        (3, 6) &         IYZY &  \{1, 3\} &  \{1, 2, 3\} &       3 &     3 \\
4     &  (0, 1, 2, 3) &         ZZII &  \{0, 1\} &     \{0, 1\} &       2 &     1 \\
4     &        (4, 5) &         IIZI &     \{2\} &        \{2\} &       1 &     0 \\
5     &        (2, 3) &         IZII &     \{1\} &        \{1\} &       1 &     0 \\
\bottomrule
\end{tabular}


==> Figs_Results/model_ham_costs_with_swaps.tex <==
\begin{tabular}{lllllrr}
\toprule
{} &      Monomial & Pauli string &    Edge & Support &  Weight &  Cost \\
Layer &               &              &         &         &         &       \\
\midrule
0     &  (0, 1, 2, 3) &         ZZII &  \{0, 1\} &  \{0, 1\} &       2 &     1 \\
     &        (4, 5) &         IIZI &     \{2\} &     \{2\} &       1 &     0 \\
     &        (6, 7) &         IIIZ &     \{3\} &     \{3\} &       1 &     0 \\
1     &        (0, 1) &         ZIII &     \{0\} &     \{0\} &       1 &     0 \\
     &        (2, 3) &         IZII &     \{1\} &     \{1\} &       1 &     0 \\
4     &        (0, 5) &         IIXX &  \{0, 2\} &  \{2, 3\} &       2 &     1 \\
     &        (2, 7) &         XXII &  \{1, 3\} &  \{0, 1\} &       2 &     1 \\
5     &        (1, 4) &         IIYY &  \{0, 2\} &  \{2, 3\} &       2 &     1 \\
     &        (3, 6) &         YYII &  \{1, 3\} &  \{0, 1\} &       2 &     1 \\
\bottomrule
\end{tabular}


==> Figs_Results/model_ham_interactions.tex <==
\begin{tabular}{ll}
\toprule
    Monomial &  Modes \\
\midrule
      (0, 1) &    \{0\} \\
(0, 1, 2, 3) & \{0, 1\} \\
      (0, 5) & \{0, 2\} \\
      (1, 4) & \{0, 2\} \\
      (2, 3) &    \{1\} \\
      (2, 7) & \{1, 3\} \\
      (3, 6) & \{1, 3\} \\
      (4, 5) &    \{2\} \\
      (6, 7) &    \{3\} \\
\bottomrule
\end{tabular}

==> Figs_Results/srvo3_data.tex <==
\begin{tabular}{lrrrr}
\toprule
                       Algorithm &  Qubits &  Interactions depth &  Swaps depth &  Circuit depth \\
\midrule
            VQE w/o swap network &     180 &                 412 &            0 &            412 \\
                             VQE &     180 &                 108 &          384 &            492 \\
TDS (prioritising circuit depth) &     180 &                 111 &          384 &            495 \\
TDS (prioritising Trotter error) &     180 &                 117 &          384 &            501 \\
\bottomrule
\end{tabular}

==> results_table.tex <==
\begin{tabular}{llllrr}
\toprule
         &    &   &         &  Qubits &  Depth \\
Material & Bands & Hop. order & Algorithm &         &        \\
\midrule
\multirow{8}{*}{GaAs} & \multirow{8}{*}{4} & \multirow{4}{*}{2} & TDS &     234 &   1489 \\
         &    &   & TDS$^*$ &     234 &   1509 \\
         &    &   & VQE &     234 &   1489 \\
         &    &   & VQE$^*$ &     234 &   1437 \\
\cline{3-6}
         &    & \multirow{4}{*}{5} & TDS &    1120 &   3361 \\
         &    &   & TDS$^*$ &    1120 &   3757 \\
         &    &   & VQE &    1120 &   3361 \\
         &    &   & VQE$^*$ &    1120 &   3676 \\
\cline{1-6}
\cline{2-6}
\cline{3-6}
\multirow{8}{*}{H$_3$S} & \multirow{8}{*}{7} & \multirow{4}{*}{2} & TDS &     396 &   2641 \\
         &    &   & TDS$^*$ &     396 &   2934 \\
         &    &   & VQE &     396 &   2641 \\
         &    &   & VQE$^*$ &     396 &   2783 \\
\cline{3-6}
         &    & \multirow{4}{*}{6} & TDS &    1870 &  15273 \\
         &    &   & TDS$^*$ &    1870 &  18901 \\
         &    &   & VQE &    1870 &  15273 \\
         &    &   & VQE$^*$ &    1870 &  17853 \\
\cline{1-6}
\cline{2-6}
\cline{3-6}
\multirow{4}{*}{Li$_2$CuO$_2$} & \multirow{4}{*}{11} & \multirow{4}{*}{8} & TDS &    1024 &   4758 \\
         &    &   & TDS$^*$ &    1024 &   6448 \\
         &    &   & VQE &    1024 &   4760 \\
         &    &   & VQE$^*$ &    1024 &   6042 \\
\cline{1-6}
\cline{2-6}
\cline{3-6}
\multirow{16}{*}{SrVO$_3$} & \multirow{8}{*}{3} & \multirow{4}{*}{2} & TDS &     180 &   1125 \\
         &    &   & TDS$^*$ &     180 &    865 \\
         &    &   & VQE &     180 &   1125 \\
         &    &   & VQE$^*$ &     180 &    865 \\
\cline{3-6}
         &    & \multirow{4}{*}{5} & TDS &     870 &   4157 \\
         &    &   & TDS$^*$ &     870 &   2633 \\
         &    &   & VQE &     870 &   4157 \\
         &    &   & VQE$^*$ &     870 &   2633 \\
\cline{2-6}
\cline{3-6}
         & \multirow{8}{*}{12} & \multirow{4}{*}{2} & TDS &     666 &   3031 \\
         &    &   & TDS$^*$ &     666 &   3750 \\
         &    &   & VQE &     666 &   3031 \\
         &    &   & VQE$^*$ &     666 &   3686 \\
\cline{3-6}
         &    & \multirow{4}{*}{4} & TDS &    3120 &  11033 \\
         &    &   & TDS$^*$ &    3120 &  19841 \\
         &    &   & VQE &    3120 &  11033 \\
         &    &   & VQE$^*$ &    3120 &  19618 \\
\bottomrule
\end{tabular}

